Minimal Actuator Selection for Linear Time Invariant Systems

Selecting a few available actuators to ensure the controllability of a linear system is a fundamental problem in control theory. Previous works either focus on optimal performance, simplifying the controllability issue, or make the system controllable under structural assumptions, such as in graphs or when the input matrix is a design parameter. We generalize these approaches to offer a precise characterization of the general minimal actuator selection problem where a set of actuators is given, described by a fixed input matrix, and goal is to choose the fewest actuators that make the system controllable. We show that this problem can be equivalently cast as an integer linear program and, if actuation channels are sufficiently independent, as a set multicover problem under multiplicity constraints. The latter equivalence is always true if the state matrix has all distinct eigenvalues, in which case it simplifies to the set cover problem. Such characterizations hold even when a robust selection that tolerates a given number of faulty actuators is desired. Our established connection legitimates a designer to use algorithms from the rich literature on the set multicover problem to select the smallest subset of actuators, including exact solutions that do not require brute-force search.

==> Sections/Introduction-arxiv.tex <==
%!TEX root = ../MinimalActuatorSelection.tex

\section{Introduction}

Ensuring controllability of a dynamical system is key to achieving regulation and desired behavior without degrading performance.
This challenge is exacerbated in modular and hierarchical systems built by interconnecting independent units,
which makes co-design tractable and robust~\cite{Zardini22cdc-modularCodesign,Incer25-Pacti}. 
As the size of the system grows, controllability becomes even more important
since strategically placing a few actuators can save costs and is practically feasible~\cite{DeLorenzo90jgcd-SensorActuatorSelection,Liu11nature-controllabilityNetworks}. So we investigate the problem of choosing the smallest subset of actuators from a given admissible set that renders the system controllable.

\subsubsection*{Related work}
The early work~\cite{VanDeWal01automatica-selectionIO} reviews approaches for the selection of sensors and actuators based on several requirements,
including binary and quantitative metrics related to observability and controllability of the state,
location of poles and zeros,
and input-output controllability.
Actuator selection has subsequently been tackled via principled optimization formulations.
A convex $\mathcal{H}_2$-optimal control problem is formulated in~\cite{Zare20tac-proximalAlgorithms} using sparsity-promoting functions to reduce the number of actuators and extended to lossy wireless networks in~\cite{Zhong24automatica-sparseSensorSelection}.
Argha~\emph{et al.} codesign actuators and control law in~\cite{Argha19ijc-optimalActuatorSensorSelection} using linear matrix inequalities (LMI).
Other structural tools, such as a balanced transformation of the Gramian matrices, have been used to select sensors and actuators~\cite{Manohar22tac-OptimalSensor}. 
Furthermore, the selection problem for optimal sensor fusion via a tractable heuristic approach~\cite{Joshi09tsp-sensorSelectionConvex}, the controller-actuator optimal codesign for LQG control~\cite{Tzoumas21tac-lqgCodesign}, and computational limitations of optimal sensor selection~\cite{Tzoumas16acc-sensorPlacementKalman} have also been investigated.
Within static actuator selection literature,
a significant body of works focuses on networked control and multi-agent systems.
Representative examples are~\cite{Guo21tac-actuatorPlacementGreedy,Pasqualetti14tcns-controllabilityMetricsNetworks,Clark12cdc-leaderSelection,Yazicioglu16tcns-graphDistancesControllability,Chapman13acc-strongStructuralControllability,Doostmohammadian20sj-driverNodes,Summers16tcns-submodularity,Baggio22ar-energyAwareControllability},\revision{\cite{Tzoumas2016tcns-minimalActuatorPlacement,Taha2017acc-actuatorSelectionCPS} where selection typically minimizes a function of the controllability Gramian or LQR/LQG control cost.
	However,
	graphs induce specific structures on the state matrix and assume that each node can be individually actuated, imposing a diagonal input matrix.}
Related to the static selection problem, significant effort has been devoted to developing time-varying schedules for performance improvement and online adaptation.
Hands-off control reduces total actuation time via $\ell_1$ regularization~\cite{Nagahara16-MaximumHands-OffControl,Ikeda21lcss-maximumHandsOffTimeSpace}.
Algorithms to design schedules in an offline~\cite{Siami21tac-actuatorScheduling} and online fashion~\cite{Vafaee24automatica-realTimeSensorSelection} have also been developed.
A recent line of work studies controllability in linear systems where at most $s$ inputs are enabled at each time~\cite{Joseph24now-sparseActuatorControl},
offering an actuator schedule design with controllability guarantee in~\cite{Ballotta24lcss-actuatorSchedulingGuarantee}.
More recently, learning-based methods with unknown dynamics have been studied in~\cite{Ye24tac-onlineActuatorSelection} to choose both actuators and inputs in LQR online, and in~\cite{Chekan24tac-learnControlSwitching} to learn the dynamics while switching, with a focus on stability.
For LQ control, a submodular optimization problem is formulated in~\cite{Chamon19cdc-actuatorScheduling}.
Nearly all works above focus on optimal performance without openly discussing how to ensure controllability, with the exception of~\cite{Tzoumas2016tcns-minimalActuatorPlacement,Guo21tac-actuatorPlacementGreedy,Clark12cdc-leaderSelection} which assume diagonal input matrix.

A complementary line of research regards controllability as a design objective.
Most relevant to the current study is
the seminal paper~\cite{Olshevsky14tcns-minimalControllability}, which formulates the minimal controllability problem (MCP). Here, the input matrix can be freely designed, and the objective is to minimize its nonzero (diagonal) elements, each representing a directly controlled state.
Research efforts have addressed robust formulations to accommodate malfunctioning and faults,
with early studies dating back to aerospace missions in the 1980s~\cite{VanderVelde84jgcd-placementControlComponentsFailures}.
Pequito~\emph{et al.}~\cite{Pequito17automatica-robustMinimalControllability} extend the setup of Olshevski~\cite{Olshevsky14tcns-minimalControllability} and include a fixed number of possible faults that disable actuators,
establishing an equivalence with the set multicover problem and adapting a greedy selection algorithm.
This formulation is extended to codesign of sensors and actuators in~\cite{Ramos21ijrnc-robustMinimalControllabilityObservability}.
However,
all elements of the input matrix are freely assigned, and its size is conservatively chosen to guarantee controllability under faults.
Zhang~\emph{et al.}~\cite{Zhang23tac-observabilityRobustnessSensorFailures} consider the opposite problems of ensuring observability when either sensors are removed, or state variables are masked out from outputs.
They prove that the former problem can be solved in polynomial time if the eigenspaces of the state matrix have bounded dimension,
in striking contrast with the MCP.
Several studies investigate the robustness of (structural) controllability in graphs under deletion of edges or nodes, modeling failure of links or actuators~\cite{Abbas25tcns-resilientControllabilityNetworks,Chen22jai-controllabilityRobustnessNetworks,Moothedath20tcns-optimalNetworkTopologyDesign,Mousavi17acc-robustStrongStructuralControllability,Pirani23automatica-GraphTheoreticApproachesResilience,Zhang19ijrnc-MinimalPerturbationsControllability}.

\subsubsection*{Contribution}
Although extensive research addresses actuator selection problems,
we identify two main limitations.
Most
existing works that select actuators from a given set mostly focus on performance without explicitly addressing controllability.
Conversely, approaches based on the MCP and its robust versions assume that the actuators can arbitrarily choose which state variables to directly act upon.
This formulation works well for leader selection in multi-agent systems or dynamics on graphs where each node is described by a (set of) state variable(s),
but it is not suited to the general case where the effect of actuators on the dynamics may not be designed,
i.e.,
when the input matrix is given.
These limitations further require a dedicated study of robust selection to tolerate faults.

We fill this gap and systematically study the \emph{minimal actuator selection} problem, where we choose the minimum number of actuators that ensure controllability of a linear time-invariant system.
First,
we show that this problem can be written as an integer linear program with no loss of generality.
Second,
we prove that,
under technical assumptions,
it is equivalent to the set multicover problem.
This reduces to the set cover problem if the state matrix has all distinct eigenvalues, analogously to the setups in~\cite{Olshevsky14tcns-minimalControllability,Pequito17automatica-robustMinimalControllability}.
Third,
we extend our formulation to the robust version, where a given number of actuators may fail, and the corresponding selected columns of the input matrix are removed.
We prove that both the ILP characterization and the equivalence with the set multicover problem remain valid and require only modifying the parameters of the problems to incorporate the actuator redundancy necessary to counterbalance faults.
Finally,
we review algorithms for selection, drawing inspiration from the rich literature on set multicover.
Notably, both polynomial-time procedures with provable suboptimality gaps and exact algorithms that avoid brute-force search are available.
This may be attractive when sufficient computing power is available,
e.g., for offline design or sporadic reconfiguration.

% \subsubsection*{Paper organization}
% We formulate the minimal actuator selection problem,
% characterize it as an ILP,
% and discuss the equivalence with set multicover in \autoref{sec:minimal-actuator-selection}.
% We address the robust formulation in \autoref{sec:robust-minimal-actuator-selection}.
% We review and compare selection algorithms from control and computer science literature in \autoref{sec:algorithms}.
% We conclude and discuss the future outlook in \autoref{sec:conclusion}.
